SATformer: Transformer-Based UNSAT Core Learning

This paper introduces SATformer, a novel Transformer-based approach for the Boolean Satisfiability (SAT) problem. Rather than solving the problem directly, SATformer approaches the problem from the opposite direction by focusing on unsatisfiability. Specifically, it models clause interactions to identify any unsatisfiable sub-problems. Using a graph neural network, we convert clauses into clause embeddings and employ a hierarchical Transformer-based model to understand clause correlation. SATformer is trained through a multi-task learning approach, using the single-bit satisfiability result and the minimal unsatisfiable core (MUC) for UNSAT problems as clause supervision. As an end-to-end learning-based satisfiability classifier, the performance of SATformer surpasses that of NeuroSAT significantly. Furthermore, we integrate the clause predictions made by SATformer into modern heuristic-based SAT solvers and validate our approach with a logic equivalence checking task. Experimental results show that our SATformer can decrease the runtime of existing solvers by an average of 21.33%.

==> bak_intro_0519.tex <==
\section{Introduction} \label{Sec:Intro}
% ====================================
% SAT problem 
% The Boolean SATisfiability (SAT) problem is one of the most fundamental problems with numerous applications in various fields. For example, solving the SAT problem has been the core of dealing with software verification~\cite{jackson2000finding}, circuit design~\cite{goldberg2001using} and AI planning~\cite{kautz1992planning}. The SAT problem is, given a propositional Boolean logic formula with several variables, determining whether there exists at least one assignment for these variables that makes the formula outputs $true$. If so, the problem instance $\phi$ is \textit{satisfiable}, otherwise \textit{unsatisfiable}. The propositional SAT instance can be transformed into various equivalent formats. Conjunctive Normal Form (CNF) is one of the most widely used formats in contemporary SAT solvers. The SAT instance represented in CNF consists of a conjunction of \textit{clauses} and each clause constructed by a disjunction of \textit{literals}. 

The Boolean Satisfiability (SAT) problem is one of the most fundamental problems in various fields. For example, solving the SAT problem has been the core of dealing with software verification~\cite{jackson2000finding}, circuit design~\cite{goldberg2001using} and AI planning~\cite{kautz1992planning}. It determines whether there exists at least one assignment for these variables that makes a given formula evaluate to $true$. 


% ====================================
% Learning-based solver 
However, the SAT problem is the first proven NP-complete problem~\cite{cook1971complexity}, and there is no solving algorithm in polynomial time. To handle the large industrial SAT instance, the prevalent modern solvers~\cite{sorensson2005minisat,BiereFazekasFleuryHeisinger,selman1993local} follow the heuristic-based searching strategies. With the emergence of deep learning, many learning-based SAT solving approaches have been studied extensively in the past few years. The learning-based approaches fall into two directions. On the one hand, learning-aided approaches try to learn an efficient heuristic and are integrated with the traditional SAT solvers~\cite{kurin2020can,zhang2020nlocalsat,selsam2019guiding}. On the other hand, the end-to-end approaches~\cite{selsam2018learning,amizadeh2018learning,ozolins2021goal,li2022deepsat} solve SAT problems from scratch in a standalone way. Generally, the performance of the end-to-end solver lags behind the learning-aided approaches by a large margin. Nevertheless, since the neural network in the learning-aided SAT solving approach is only a plug-in component, the upper-bound performance of learning-aided solvers is limited by the corresponding backbone solvers. In contrast, end-to-end approaches provide a potential way to improve the efficiency of SAT solving by fundamentally breaking such an upper bound. In this work, we focus on boosting the performance of the end-to-end learning approaches.

% ====================================
% Our observation: UNSAT core
% The propositional SAT instance can be transformed into various equivalent formats. Conjunctive Normal Form (CNF) is one of the most widely used formats in contemporary SAT solvers. The SAT instance represented in CNF consists of a conjunction of \textit{clauses} and each clause constructed by a disjunction of \textit{literals}. Usually, the learning-based end-to-end SAT solvers \cite{selsam2018learning, amizadeh2018learning, ozolins2021goal} ignore the interaction among clauses. Different from the previous approaches, we start from a novel perspective by modeling the relationship among clauses. Specifically, there must be at least one subset of clauses named Unsatisfiable Core (UNSAT Core) that causes the constituted sub-problem to be unsatisfiable. The SAT instance will be inferred as unsatisfiable if and only if there exists an UNSAT core. Therefore, the solving procedure can be considered as modeling the relationship among clauses and determining whether an UNSAT core can be derived from the original instance. 

% 整体逻辑是先说他们用了啥监督信号，但是忽略了sat/unsat的本质，说出mus的概念，然后motivate 我们去做这样一件事情
% In particular, NeuroSAT considers from the instance level and ignores the essence of satisfiability, i.e., a satisfying variable assignment can be found when searching all possible assignments. 
Among end-to-end SAT solvers, NeuroSAT~\cite{selsam2018learning} models the SAT problem as a classification task and trains a classifier only with single-bit supervision (satisfiable or not). However, the instance level supervision is relatively weak for the model training. DG-DAGRNN~\cite{amizadeh2018learning} and DeepSAT~\cite{li2022deepsat} target on the circuit satisfiability problem. They leverage the structure information of the circuit rather than the uniform Boolean formula expression in conjunctive normal form (CNF). 
% DG-DAGRNN~\cite{amizadeh2018learning} introduces a reinforcement learning approach to maximize the score leading to satisfiability. DeepSAT~\cite{li2022deepsat} formulates the SAT solution as a produce of conditional Bernoulli distributions and obtains assignment by maximizing the joint probability. Yet, these approaches all require evaluating assignment for multiple times. 
Different from the previous approaches, we take CNF instance as inputs and start from the inverse proposition of Boolean satisfiability, i.e., unsatisfiability. In the searching-based solving algorithm, the solver asserts the instance to be unsatisfiable if and only if an unavoidable \textit{conflict} exists when exploring the satisfying assignment. This conflict is reflected in a subset of clauses, named Unsatisfiable Core (UNSAT Core). Specifically, the sub-problem constituted by the UNSAT core is still unsatisfiable. Therefore, the solving procedure can be considered as modeling the interaction among the clauses and determining whether an UNSAT core can be discovered from the original instance. 

% ====================================
% Our method 
In this paper, we present \textit{SATformer}, a Transformer-based SAT solving approach guided by the UNSAT cores.  
Firstly, to differentiate the clauses involved in the UNSAT core, our model applies a graph neural network (GNN) to obtain the clause embeddings and learns a probability distribution of clauses to formulate the contribution to unsatisfiability. Since the unsatisfiable instance does not contain only a single UNSAT core, we take the minimal unsatisfiable core (MUC) as supervision (similar to NeuroCore~\cite{selsam2019guiding}), which has less uncertainty. 

% Secondly, as a set of clauses may lead to unsatisfiability, our model determines the satisfiability by learning the clause interactions. 
Secondly, as a set of clauses may construct an UNSAT core, satisfiability solving can be realized by modeling the clause interactions. To this end, we equip the Transformer blocks to draw the connection between clauses. With the guidance from UNSAT core prediction, our model can learn to assign higher attention weight to these key clauses causing unsatisfiable. 

Thirdly, the self-attention mechanism of the plain Transformer only learns pairwise dependency. To accommodate the requirements of modeling multiple clauses, we design a hierarchical Transformer structure. Our model merges clauses into clause groups level by level and captures the relationships between a pair of clause groups with various scales. 

The experimental results indicate that our proposed model is competitive with previous end-to-end SAT solvers. We also prove that after classifying clauses into two categories: likely and unlikely to form an UNSAT core, the effectiveness of our SATformer comes from focusing on these clauses tending to form an UNSAT core. 

% ====================================
% Contribution
The contributions of this work are summarized as follows: 
\begin{itemize}
    \item We model the learning-based SAT solving from a novel perspective. In particular, we design a Transformer-based model to capture the correlation among clauses and determine whether the instance is satisfiable or not. 
    \item We apply the minimal UNSAT core as significant clause-level supervision. Our proposed model distinguishes clauses as \textit{likely} or \textit{unlikely} to form an UNSAT core. Moreover, the Transformer blocks inside our model pays much attention to these important clauses with core-guided. 
    \item We propose a hierarchical Transformer structure to package clauses. Therefore, our model can model relationships from different granularities, instead of pair relationships between clauses. 
\end{itemize}

% We organize the remaining sections as follows. The background of SAT problem and some related work are summarized in Sec.~\ref{Sec:Related}. The detailed architecture and methodology of our SATformer are elaborated in Sec.~\ref{Sec:Method}. Sec.~\ref{Sec:Exp} compares our approach with other end-to-end learning-based SAT solvers and proves the effectiveness of our design. Sec.~\ref{Sec:Conclusion} concludes this paper.  

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


==> bak_intro_0523.tex <==
\section{Introduction} \label{Sec:Intro}
% ====================================
% SAT problem 
% The Boolean SATisfiability (SAT) problem is one of the most fundamental problems with numerous applications in various fields. For example, solving the SAT problem has been the core of dealing with software verification~\cite{jackson2000finding}, circuit design~\cite{goldberg2001using} and AI planning~\cite{kautz1992planning}. The SAT problem is, given a propositional Boolean logic formula with several variables, determining whether there exists at least one assignment for these variables that makes the formula outputs $true$. If so, the problem instance $\phi$ is \textit{satisfiable}, otherwise \textit{unsatisfiable}. The propositional SAT instance can be transformed into various equivalent formats. Conjunctive Normal Form (CNF) is one of the most widely used formats in contemporary SAT solvers. The SAT instance represented in CNF consists of a conjunction of \textit{clauses} and each clause constructed by a disjunction of \textit{literals}. 

The Boolean Satisfiability (SAT) problem involves determining whether there exists at least one assignment for a set of variables that makes a given Boolean formula to be $true$. This problem is one of the most fundamental problems in various fields, particularly in electronic design automation (EDA). Solving the SAT problem is crucial for dealing with logic equivalence checking (LEC)\cite{goldberg2001using}, model checking\cite{mcmillan2003interpolation}, and automatic test pattern generation (ATPG)\cite{yang2004trangen}. Since the SAT problem is the first proven NP-complete problem\cite{cook1971complexity}, there exists no algorithm to completely solve it in polynomial time. 
To handle large industrial SAT instances, modern solvers~\cite{sorensson2005minisat,BiereFazekasFleuryHeisinger,selman1993local} use heuristics-based searching techniques that return a \textit{satisfiable} (SAT) response if a valid assignment is found, an \textit{unsatisfiable} (UNSAT) response if no valid assignment is found after exhausting all searching paths, or an \textit{unknown} response if the maximum runtime is exceeded. 

Although existing solvers have demonstrated promising results on general benchmarks~\cite{lu2003circuit, audemard2009glucose, audemard2018glucose}, there are still some limitations hindering their solving ability for EDA problems. 
% 一方面现有的启发式不会预估实例的可满足性选择合适的策略。根据~\cite{huang2022neural}中的观察，efficiency of the same heuristics can vary greatly on solving different kinds of instances from ATPG tasks. For instance, local search heuristic~\cite{hoos2000local} can reduce the runtime for solving SAT instances, while it increases the runtime for solving UNSAT instances significantly. 与之相反，dynamic restart heuristic~\cite{biere2008adaptive}能够在UNSAT instances上表现更好，但在SAT instances上效果欠佳。由于求解器会prove SAT and UNSAT in different ways~\cite{oh2015between}，错误地配置求解器启发式策略甚至会增加50\%的求解时间~\cite{gagliolo2010algorithm}. 即使现代求解器集成了适用于SAT或UNSAT问题的求解模式，但均需要用户手动选择，而不是在求解前自动预测问题实例的可满足性。% 因此，在执行求解过程前快速判断当前实例的可满足性，并选择satisfiability-oriented heuristic有希望进一步降低求解时间。
% On the one hand, existing heuristics cannot predict the satisfiability of instances before solving. According to observations in~\cite{huang2022neural}, the same heuristics can vary greatly in efficiency when solving SAT and UNSAT instances in ATPG tasks. For example, the local search heuristic~\cite{hoos2000local} can reduce the runtime for solving SAT instances but significantly increase the runtime for solving UNSAT instances. Conversely, the dynamic restart heuristic~\cite{biere2008adaptive} performs better on UNSAT instances but does not perform well on SAT instances. Configuring solver heuristics inappropriately can even increase the solving time by 50\%~\cite{gagliolo2010algorithm}, due to the fact that solvers prove SAT and UNSAT in different ways~\cite{oh2015between}. While modern solvers~\cite{cadical, queue2019cadical, fleury2020cadical, audemard2018glucose} integrate SAT solving mode and UNSAT solving mode, they require manual selection without predicting the satisfiability on their own.

On the one hand, existing solvers lack ability to guide heuristic selection based on the satisfiability. Although modern solvers~\cite{cadical, queue2019cadical, fleury2020cadical, audemard2018glucose} support configuring the satisfiability-specific mode (SAT mode or UNSAT mode), they still require manual choice rather than predicting satisfiability on their own. Furthermore, the same heuristics can exhibit significant variations in efficiency when solving SAT and UNSAT instances in ATPG tasks, as observed in~\cite{huang2022neural}. For example, the local search heuristic~\cite{hoos2000local} can reduce the runtime for solving SAT instances, while significantly increasing the runtime for solving UNSAT instances. Conversely, the dynamic restart heuristic~\cite{biere2008adaptive} can speed up solving UNSAT instances but does not perform well on SAT instances. Configuring solver heuristics inappropriately can even increase the solving time by 50\%~\cite{gagliolo2010algorithm}, due to the fact that solvers prove SAT and UNSAT in different ways~\cite{oh2015between}. Therefore, predicting SAT or UNSAT before solving is essential for heuristic adjustment and to maximize the effectiveness of heuristic algorithms in solvers. 

% 另一方面，已有的启发式策略用于求解UNSAT问题的效果不佳。由于EDA任务中UNSAT实例求解极其困难，这使得在实际EDA应用中，求解器在证明问题不可满足上需要消耗大量时间。To be specific, ATPG engines spend most of run time in proving that a fault is untestable~\cite{liang1995identifying, heragu1997fast} and logic synthesis engines 在验证两个电路逻辑等价（两个电路通过XOR门组合成的miter电路不可满足）上耗时明显~\cite{goldberg2003verification, mishchenko2006improvements}。% 因此，一种针对UNSAT问题求解的启发式能够有效提升EDA工具中求解器的效率。

On the other hand, existing solvers lack of dedicated heuristics for UNSAT problems. In practical EDA applications, tools often need to solve numerous UNSAT problems, which are more challenging than SAT problems.
For example, in logic equivalence checking and model checking, the majority of instances are unsatisfiable and require significant runtime to prove the unsatisfiability~\cite{goldberg2003verification, mishchenko2006improvements}. 
Similarly, in ATPG, a substantial amount of runtime is required to prove that some faults are untestable, which corresponds to proving unsatisfiability using a solver~\cite{liang1995identifying, heragu1997fast}. Therefore, incorporating an efficient UNSAT heuristic can significantly improve the generalizability and efficiency of modern solvers in the EDA field. 

To address the above issues, we propose \textit{SATformer}, a Boolean satisfiability solving framework that predicts satisfiability and also speeds up solving process for unsatisfiable problems. 
Firstly, We rethink the essence of unsatisfiability as the existence of an unsatisfiable sub-problem, and then propose to deal with UNSAT problem by modeling clause interaction. 
Specifically, the solver asserts that the instance is unsatisfiable if and only if an unavoidable conflict arises while searching for valid assignments. This conflict is reflected in a subset of clauses known as the Unsatisfiable Core (UNSAT Core), where the sub-problem constituted by the UNSAT core is also unsatisfiable. Therefore, by capturing the interaction among clauses and discovering the UNSAT core, we can determine the satisfiability of the given instance.

Secondly, to model the correlation among clauses, we design a deep learning model that represents clauses as embeddings using a graph neural network (GNN) and captures the connections among clauses by using a novel hierarchical Transformer-based model. To be specific, the hierarchical model merges clauses into clause groups level by level and captures the relationships between two clause groups. In that case, our novel Transformer-based model can learn the interaction among multiple clauses, instead of just the pairwise dependency as in the standard Transformer. Besides, our model is trained with two tasks: satisfiability prediction with a single-bit supervision, and the UNSAT Core prediction supervised by the minimal unsatisfiable core (MUC). The core with the minimal number of clauses has less diversity, despite the possibility of an UNSAT instance containing multiple cores of varying size, as noted in NeuroCore~\cite{selsam2019guiding}. 

% We further propose a hierarchical Transformer-based model and a multi-task training strategy to model problem instances effectively. On the one hand, since the self-attention mechanism of the standard Transformer only learns pairwise dependency, we design a hierarchical Transformer structure that merges clauses into clause groups level by level and captures the relationships between pairs of clause groups at different scales. On the other hand, our model is trained with two tasks: satisfiability prediction with a single-bit supervision, and the UNSAT Core prediction supervised by the minimal unsatisfiable core (MUC). As noted in NeuroCore~\cite{selsam2019guiding}, the core with the minimal number of clauses has less diversity, despite the possibility of an UNSAT instance containing multiple cores of varying size. Moreover, MUC is the much easier UNSAT sub-problem to prove~\cite{nadel2010boosting}. 

Thirdly, we introduce SATformer as an initialization heuristic for SAT solvers. Our SATformer produces a binary prediction indicating the satisfiability and a \textit{prediction score} for each clause indicating the probability of forming UNSAT core. Clauses with high prediction scores are considered more contributive to unsatisfiability. Therefore, solving sub-problems composed of high-score clauses can lead to UNSAT results more quickly. We apply the clause prediction score to determine the searching priorities. Specifically, we calculate the corresponding priority score of variables based on the variable-clause connections and employ it as the initial variable activity score, such as Variable State Independent Decaying Sum (VSIDS)~\cite{moskewicz2001chaff}. As most SAT solvers reserve the variable branching priority interface~\cite{moskewicz2001chaff, sorensson2005minisat, queue2019cadical, fleury2020cadical}, SATformer can be flexibly integrated into them as a plug-in without much effort on solver reconstruction. Different from the previous variable branching heuristics that only focus on variable activity, our approach utilizes the correlation at the clause level. We demonstrate the effectiveness of SATformer by boosting the performance of two modern SAT solvers: CaDiCal~\cite{queue2019cadical} and Kissat~\cite{fleury2020cadical}. 

The contributions of this work are summarized as follows: 
\begin{itemize}
    \item We consider the unsatisfiability solving problem from a novel perspective, which models the correlation among clauses and identifies the existence of unsatisfiable sub-problem. 
    \item We design a hierarchical Transformer-based model to capture clause interactions. We use the minimal UNSAT core as significant clause-level supervision and train our model to distinguish clauses as \textit{likely} or \textit{unlikely} to form an UNSAT core. 
    \item We incorporate the proposed model as a learning-aided initialization heuristic into modern SAT solvers. The experimental results indicate that our model significantly speed up the solving procedure. 
\end{itemize}

We organize the paper as follows. Section~\ref{Sec:Related} reviews the related works about learning-aided SAT solvers and Transformer blocks. We propose our SATformer framework in Section~\ref{Sec:Method} and investigate the effectiveness of our model in Section~\ref{Sec:Exp}. Finally, Section~\ref{Sec:Conclusion} concludes this paper. 





%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%



% % ====================================
% % Solver heuristic 
% Although the existing heuristics demonstrate promising results, they do not guarantee to accelerate the solving process for any instances~\cite{lu2003circuit, audemard2009glucose, audemard2018glucose}. For example, the heuristic~\cite{lu2003circuit} tending to cause searching conflict can accelerate solving for unsatisfiable cases, but the speedup is not significant for satisfiable cases. This is because solvers prove SAT and UNSAT in different ways, as surveyed in \cite{oh2015between}. Moreover, in practical applications, there is usually an expectation of what results will be produced, e.g., the majority of SAT calls for hardware/software testing are satisfiable calls, while the most of SAT calls for SAT-sweep in logic synthesis are unsatisfiable calls. Therefore, assuming the satisfiability of a problem before solving and using a solver equipped with the satisfiability-oriented heuristic for justification is a feasible and efficient solving paradigm.


% \begin{wraptable}{l}{0.255\textwidth}
% \centering 
% \begin{minipage}{4.8cm}
% \small{
% \caption{Performance of SAT's Heuristics }
% \label{table:base_test}
% \resizebox{\textwidth}{14mm}{
% \begin{tabular}{|c|c|c|c|c|c|c|}
% \hline
% \multirow{2}{*}{Fault} & \multirow{2}{*}{Testability} & \multicolumn{2}{|c|}{Local Search}& \multicolumn{2}{|c|}{Restart }\\
% \cline{3-6}  
% & & On & Off & Static & Dynamic \\
% \hline
%  f1  &  Testable & 212 &  572 & 284 & 592  \\
% \hline 
%  f2  & Testable & 260 &  411  & 251 & 438  \\
% \hline
% f3  &  Testable & 488 &  713  & 473  &  821  \\
% \hline
%  f4 &  Testable & 214 & 649  & 523  & 731   \\
% \hline
% f5  &  Untestable & 2268 &  452 & 1112 & 126 \\
% \hline
% f6   & Untestable & 1546  & 112  & 1428  & 89 \\
% \hline
% f7  & Untestable & 826 &  165 & 1042 & 104 \\
% \hline
%  f8  & Untestable & 1311 & 423   &  1971 &  121 \\
% \hline 
% \end{tabular}}}
% \end{minipage}
% \end{wraptable} 

% \huilingzhen{In practice, efficiency of the same heuristics can vary greatly on solving different kinds of faults. Take $b19$ from ITC'99 as an example. We compare the effects of two conventional heuristics in CADICAL2021}~\cite{cadical}, \huilingzhen{ i.e., the local search and restart, on solving efficiency. Apart from these two heuristics, we do not change any default settings. The results are given in Table~I}. \huilingzhen{We randomly select four testable faults and four untestable faults. The runtime to solve the selected faults when turning local search on and off is given in 4th and 5th columns, and the results of static restart strategy and dynamic strategy is respectively in the 6th and 7th columns. Hereby, the static restart strategy is with a fixed frequency, while the dynamic one is with an exponential moving average heuristics}~\cite{cadical}. \huilingzhen{Table~I shows that local search can reduce the runtime for solving testable faults (i.e., SAT instances), while it increases the runtime for solving untestable faults (i.e., UNSAT instances) significantly. Different from the local search, the dynamic restart strategy can work better for untestable faults, while it increases the runtime for testable faults. The comparison also shows that the wrong settings on restart and local search can result in more than $50\%$ decrease in solving efficiency. }

% Following this direction, we propose \textit{SATformer}, a Boolean satisfiability solving framework to predict the satisfiability and speed up solving process for unsatisfiable problems. Firstly, we rethink the UNSAT problems and formulate the UNSAT problem as to determine the existence of an unsatisfiable sub-problem by modeling clause interaction. To be specific, the solver asserts the instance to be unsatisfiable if and only if an unavoidable conflict exists during exploring the valid assignment. Such conflict is reflected in a subset of clauses, named Unsatisfiable Core (UNSAT Core), where the sub-problem constituted by the UNSAT core is still unsatisfiable. Therefore, by capturing the interaction among clauses and discovering UNSAT core, we can determine the satisfiability of the given instance. 

% Secondly, to model correlation among clauses, we design a deep learning model which tokenizes clauses by a graph neural network (GNN) and draw the connections between clause tokens by Transformer blocks. We further propose a hierarchical Transformer structure and a multiple-task training strategy to model problem instances effectively. On the one hand, since the self-attention mechanism of the plain Transformer only learns pairwise dependency, we design a hierarchical Transformer structure, which merges clauses into clause groups level by level and captures the relationships between a pair of clause groups with various scales. On the other hand, our model is trained with two tasks: classifying the satisfiability and predicting which clauses are belonging to UNSAT core. Since the unsatisfiable instance does not contain only a single UNSAT core, we take the minimal unsatisfiable core (MUC) with less uncertainty as the latter supervision (similar to NeuroCore~\cite{selsam2019guiding}). 

% Thirdly, we introduce SATformer as an initialization heuristic for SAT solvers. A clause with high prediction score is likely to form a minimal unsatisfiable core, and solving sub-problems composed of clauses with high scores can lead to faster UNSAT results. Therefore, we formulate the clause prediction results of SATformer as the searching priorities. We calculate the corresponding priority score of variables based on the variable-clause connections and employ such score as the initial variable activity score, such as Variable State Independent Decaying Sum (VSIDS)~\cite{moskewicz2001chaff}. As most SAT solvers reserve the variable branching priority interface~\cite{moskewicz2001chaff, sorensson2005minisat, queue2019cadical, fleury2020cadical}, SATformer can be flexibly intergrated with them as a plug-in without much effort on solver reconstruction. Different from the previous variable branching heuristics that only focus on variable activity, our approach utilizes the correlation at the clauses level. We demonstrate the effectiveness of our SATformer by boosting two modern SAT solvers: CaDiCal~\cite{queue2019cadical} and Kissat~\cite{fleury2020cadical}. 

% The contributions of this work are summarized as follows: 
% \begin{itemize}
%     \item We consider the unsatisfiability solving problem from a novel perspective, which models the correlation between clauses and identifies the existence of unsatisfiable sub-problem. 
%     \item We design a Transformer-based model to capture clause interactions. We apply the minimal UNSAT core as significant clause-level supervision. Our proposed model distinguishes clauses as \textit{likely} or \textit{unlikely} to form an UNSAT core. 
%     \item We equip the proposed model into modern SAT solvers as a learning-aided initialization heuristic. The experimental results indicates that our model can significantly speed up solving procedure. 
% \end{itemize}

% We organize the paper as follows. Section~\ref{Sec:Related} reviews the related works about learning-aided SAT solvers and Transformer blocks. We propose our SATformer framework in Section~\ref{Sec:Method} and investigate the effectiveness of our model in Section~\ref{Sec:Exp}. Finally, Section~\ref{Sec:Conclusion} concludes this paper. 

